Invariant Smoothing on Lie Groups

In this paper we propose a (non-linear) smoothing algorithm for group-affine observation systems, a recently introduced class of estimation problems on Lie groups that bear a particular structure. As most non-linear smoothing methods, the proposed algorithm is based on a maximum a posteriori estimator, determined by optimization. But owing to the specific properties of the considered class of problems, the involved linearizations are proved to have a form of independence with respect to the current estimates, leveraged to avoid (partially or sometimes totally) the need to relinearize. The method is validated on a robot localization example, both in simulations and on real experimental data.

==> Images/figure5.tex <==
\pgfplotsset{
  	log x ticks with fixed point/.style={
  		xticklabel={
  			\pgfkeys{/pgf/fpu=true}
  			\pgfmathparse{exp(\tick)}%
  			\pgfmathprintnumber[fixed relative, precision=3]{\pgfmathresult}
  			\pgfkeys{/pgf/fpu=false}
  		}
  	},
  	log y ticks with fixed point/.style={
  		yticklabel={
  			\pgfkeys{/pgf/fpu=true}
  			\pgfmathparse{exp(\tick)}%
  			\pgfmathprintnumber[fixed relative, precision=2]{\pgfmathresult}
  			\pgfkeys{/pgf/fpu=false}
  		}
  	}
  }
  
  
  \begin{tikzpicture}[]
  \begin{loglogaxis}[height=4.5cm, 
  width=8cm, 
  enlarge x limits=false, 
  xlabel=$\sigma^2$, 
  ylabel= position RMSE, 
  log y ticks with fixed point,
%  title =,
%  legend entries={invariant,IEKF,LUKF}, 
  legend style={font=\tiny}, 
  legend columns=1, 
  legend pos= north west, 
  label style={font=\small},
  grid=both, 
  ticks=both,
  ytick = {0.01,0.1},
  xlabel style={xshift=-0ex,yshift=0.2cm}],
  \addplot+[mark=none, draw = blue] table[x=sigma,y=is] {positionrmse.txt};
%  \addplot [color=blue] table[x expr=\coordindex, y=is] \rmseposun;
%  \addplot [color=blue] table[x expr=\coordindex, y=forster] \rmseposun;
%  \addplot [color=blue] table[x expr=\coordindex, y=grissetti] \rmseposun;
%  \addplot [color=blue] table[x expr=\coordindex, y=iekf] \rmseposun;
%  \addplot [color=blue] table[x expr=\coordindex, y=lukf] \rmseposun;      
  \end{loglogaxis}
 \end{tikzpicture}


 %copier coller et changer y label pour l'orientation

   
